Automating dipole subtraction for QCD NLO calculations

In this publication the construction of an automatic algorithm to subtract infrared divergences in real QCD corrections through the Catani-Seymour dipole subtraction method [arXiv:hep-ph/9605323] is reported. The resulting computer code has been implemented in the matrix element generator AMEGIC++ [arXiv:hep-ph/0109036]. This will allow for the automatic generation of dipole subtraction terms and their integrals over the one-parton emission phase space for any given process. If the virtual matrix element is provided as well, this then directly leads to an NLO QCD parton level event generator.

==> abstract.tex <==
\abstract{%
The Catani-Seymour dipole subtraction method and it's implementation
in the code AMEGIC is described. 
The new implementation will allow an automatic generation of dipole 
subtraction terms as well as finite parts of the subtraction
terms integrated over the one parton emission phase space 
for any given process. If the virtual matrix element can be provided 
this directly allows to generate NLO QCD parton level events. 
}
